A novel multi-layer modular approach for real-time fuzzy-identification of gravitational-wave signals

Advanced LIGO and Advanced Virgo ground-based interferometers are instruments capable to detect gravitational wave signals exploiting advanced laser interferometry techniques. The underlying data analysis task consists in identifying specific patterns in noisy timeseries, but it is made extremely complex by the incredibly small amplitude of the target signals. In this scenario, the development of effective gravitational wave detection algorithms is crucial. We propose a novel layered framework for real-time detection of gravitational waves inspired by speech processing techniques and, in the present implementation, based on a state-of-the-art machine learning approach involving a hybridization of genetic programming and neural networks. The key aspects of the newly proposed framework are: the well structured, layered approach, and the low computational complexity. The paper describes the basic concepts of the framework and the derivation of the first three layers. Even if the layers are based on models derived using a machine learning approach, the proposed layered structure has a universal nature. Compared to more complex approaches, such as convolutional neural networks, which comprise a parameter set of several tens of MB and were tested exclusively for fixed length data samples, our framework has lower accuracy (e.g., it identifies 45% of low signal-to-noise-ration gravitational wave signals, against 65% of the state-of-the-art, at a false alarm probability of $10^{-2}$), but has a much lower computational complexity and a higher degree of modularity. Furthermore, the exploitation of short-term features makes the results of the new framework virtually independent against time-position of gravitational wave signals, simplifying its future exploitation in real-time multi-layer pipelines for gravitational-wave detection with new generation interferometers.

==> bibliography_gw_20210528.tex <==
%%
%% LaTeX bibliography (28/05/2021)
%% created by Daniele Dell'Aquila
%%

@article{Aartsen20,
	author = {M.G. Aartsen and others},
	journal = {Astrophys. J. Lett.},
	volume = {898},
	pages = {L10},
	year = {2020}
}

@article{Aasi15,
	author = {J. Aasi and others},
	journal = {Class. Quant. Grav.},
	volume = {32},
	pages = {074001},
	year = {2015}
}

@article{Abbott16,
	author = {B.P. Abbott and others},
	journal = {Phys. Rev. Lett.},
	volume = {116},
	pages = {061102},
	year = {2016}
}

@article{Abbott16b,
	author = {B.P. Abbott and others},
	journal = {Phys. Rev. Lett.},
	volume = {116},
	pages = {221101},
	year = {2016}
}

@article{Abbott16c,
	author = {B.P. Abbott and others},
	journal = {Phys. Rev. Lett.},
	volume = {116},
	pages = {241102},
	year = {2016}
}

@article{Abbott16d,
	author = {B.P. Abbott and others},
	journal = {Phys. Rev. Lett.},
	volume = {116},
	pages = {131103},
	year = {2016}
}

@article{Abbott16e,
	author = {B.P. Abbott and others},
	journal = {Phys. Rev. X},
	volume = {6},
	pages = {041015},
	year = {2016}
}

@article{Abbott16f,
	author = {B.P. Abbott and others},
	journal = {Living Rev. Relativity},
	volume = {19},
	pages = {1},
	year = {2016}
}

@article{Abbott16g,
	author = {T. Abbott and others},
	journal = {(Dark Energy Survey Collaboration) Mon. Not. R. Astron. Soc.},
	volume = {460},
	pages = {1270},
	year = {2016}
}

@article{Abbott17,
	author = {B.P. Abbott and others},
	journal = {(LIGO Scientific Collaboration and Virgo Collaboration), Phys. Rev. Lett.},
	volume = {119},
	pages = {161101},
	year = {2017}
}

@article{Abbott17b,
	author = {B.P. Abbott and others},
	journal = {(LIGO Scientific Collaboration and Virgo Collaboration), Astrophys. J. Lett.},
	volume = {851},
	pages = {L35},
	year = {2017}
}

@article{Abbott17c,
	author = {B.P. Abbott and others},
	journal = {(LIGO Scientific Collaboration and Virgo Collaboration), Phys. Rev. Lett.},
	volume = {119},
	pages = {141101},
	year = {2017}
}

@article{Abbott17d,
	author = {B.P. Abbott and others},
	journal = {Astrophys. J.},
	volume = {848},
	pages = {L12},
	year = {2017}
}

@article{Abbott17e,
	author = {B.P. Abbott and others},
	journal = {Astrophys. J. Lett.},
	volume = {848},
	pages = {L13},
	year = {2017}
}

@article{Abbott19,
	author = {B.P. Abbott and others},
	journal = {(LIGO Scientific Collaboration and Virgo Collaboration), Phys. Rev. X},
	volume = {9},
	pages = {031040},
	year = {2019}
}

@article{Abbott19b,
	author = {B.P. Abbott and others},
	journal = {Astrophys. J. Lett.},
	volume = {882},
	pages = {L24},
	year = {2019}
}

@article{Abbott20,
	author = {R. Abbott and others},
	journal = { (LIGO Scientific Collaboration and Virgo Collaboration), Phys. Rev. Lett.},
	volume = {125},
	pages = {101102},
	year = {2020}
}

@article{Abdo13,
	author = {A.A. Abdo and others},
	journal = {Astrophys. J. Suppl. Ser.},
	volume = {208},
	pages = {17},
	year = {2013}
}

@article{Abe18,
	author = {K. Abe and others},
	journal = {Astrophys. J. Lett.},
	volume = {857},
	pages = {L4},
	year = {2018}
}

@article{Acernese15,
	author = {F. Acernese and others},
	journal = {Class. Quant. Grav.},
	volume = {32},
	pages = {024001},
	year = {2015}
}

@article{Adams16,
	author = {T. Adams and others},
	journal = {Class. Quant. Grav.},
	volume = {33},
	pages = {175012},
	year = {2016}
}

@article{AdrianMartinez07,
	author = {S. Adri\'an-Martinez and others},
	journal = {(The ANTARES collaboration, the LIGO scientific collaboration and	the Virgo collaboration) J. Cosm. Astropart. Phys.},
	volume = {6},
	pages = {008},
	year = {2007}
}

@article{Allen12,
	author = {B. Allen and W.G. Anderson and P.R. Brady and D.A. Brown and J.D.E. Creighton},
	journal = {Phys. Rev. D},
	volume = {85},
	pages = {122006},
	year = {2012}
}

@article{Babak13,
	author = {S. Badak and others},
	journal = {Phys. Rev. D},
	volume = {87},
	pages = {024033},
	year = {2013}
}

@article{Baker06,
	author = { J. G. Baker and others},
	journal = {Phys. Rev. Lett.},
	volume = {96},
	pages = {111102},
	year = {2006}
}

@article{Blanchet98,
	author = {Luc Blanchet},
	journal = {Class. Quant. Grav.},
	volume = {15},
	pages = {1971},
	year = {1998}
}

@article{Blanchet04,
	author = {Blanchet and others},
	journal = {Phys. Rev. Lett.},
	volume = {93},
	pages = {091101},
	year = {2004}
}


@article{Blanchet02,
	author = {Blanchet and others},
	journal = {Phys. Rev. D},
	volume = {65},
	pages = {061501(R)},
	year = {2002}
}

@article{Buccheri21,
	author = {E. Buccheri and D. Dell'Aquila and M. Russo},
	journal = {Diab. Res. Clin. Pract.},
	volume = {174},
	pages = {108722},
	year = {2021}
}

@article{Buccheri22,
	author = {E. Buccheri and D. Dell'Aquila and M. Russo},
	journal = {Obes. Medicine},
	volume = {31},
	pages = {100398},
	year = {2022}
}

@article{Campanelli06,
	author = {M. Campanelli and others},
	journal = {Phys. Rev. D},
	volume = {96},
	pages = {111101},
	year = {2006}
}

@article{Campobello20,
	author = {G. Campobello and D. Dell'Aquila and M. Russo and A. Segreto},
	journal = {Applied Soft Comp.},
	volume = {94},
	pages = {106488},
	year = {2020}
}

@article{Chatterji04,
	author = {S. Chatterji and others},
	journal = {Class. Quant. Grav.},
	volume = {21},
	pages = {S1809},
	year = {2004}
}

@article{DellAquila21,
	author = {D. Dell'Aquila and M. Russo},
	journal = {Comp. Phys. Comm.},
	volume = {259},
	pages = {107667},
	year = {2021}
}

@article{DellAquila23,
	author    = {D. Dell'Aquila and B. Gnoffo and I. Lombardo and F. Porto and M. Russo},
	journal   = {Jour. Phys. G.: Nucl. Part. Phys.},
	volume    = {50},
	pages     = {015101},
	year      = {2023}
}

@article{Gabbard18,
	author = {H. Gabbard and others},
	journal = {Phys. Rev. Lett.},
	volume = {120},
	pages = {141103},
	year = {2018}
}

@article{George18,
	author = {D. George and E.A. Huerta},
	journal = {Phys. Lett. B},
	volume = {778},
	pages = {64},
	year = {2018}
}

@article{George18b,
	author = {D. George and E.A. Huerta},
	journal = {Phys. Rev. D},
	volume = {97},
	pages = {044039},
	year = {2018}
}

@article{giannakopoulos2015pyaudioanalysis,
	title={pyAudioAnalysis: An Open-Source Python Library for Audio Signal Analysis},
	author={Giannakopoulos, Theodoros},
	journal={PloS one},
	volume={10},
	number={12},
	year={2015},
	publisher={Public Library of Science}
}

@article{Husa16,
	author = {S. Husa and others},
	journal = {Phys. Rev. D},
	volume = {93},
	pages = {044006},
	year = {2016}
}

@article{Indik18,
	author = {N. Indik and others},
	journal = {Phys. Rev. D},
	volume = {97},
	pages = {124008},
	year = {2018}
}

@article{Khan16,
	author = {S. Khan and others},
	journal = {Phys. Rev. D},
	volume = {93},
	pages = {044007},
	year = {2016}
}

@article{Kidder08,
	author = {L. E. Kidder},
	journal = {Phys. Rev. D},
	volume = {77},
	pages = {044016},
	year = {2008}
}

@article{Klimenko08,
	author = {S. Klimenko and others},
	journal = {Class. Quant. Grav.},
	volume = {25},
	pages = {114029},
	year = {2008}
}

@article{Klimenko16,
	author = {S. Klimenko and others},
	journal = {Phys. Rev. D},
	volume = {93},
	pages = {042004},
	year = {2016}
}

@book{Koza92,
	title = {Genetic Programming: On the Programming of Computers by Means of Natural Selection},
	author = {John R. Koza},
	year = {1992}, 
	publisher = {MIT Press, Cambridge, MA, USA}
}

@misc{lalsuite,
	author         = "{LIGO Scientific Collaboration}",
	title          = "{LIGO} {A}lgorithm {L}ibrary - {LALS}uite",
	howpublished   = "free software (GPL)",
	doi            = "10.7935/GT1W-FZ16",
	year           = "2018"
}

@article{Li12,
	author = {T.G.F. Li and others},
	journal = {Phys. Rev. D},
	volume = {85},
	pages = {082003},
	year = {2012}
}

@misc{LIGOT1800044,
	author = {L. Barsotti and S. Gras and M. Evans and P. Fritschel},
	title = {Technical note: LIGO-T1800044, The updated Advanced LIGO design curve},
	url = {https://dcc.ligo.org/T1800044-v5}
}

@article{Mishra10,
	author = {C.K. Mishra and others},
	journal = {Phys. Rev. D},
	volume = {82},
	pages = {064010},
	year = {2010}
}

@article{Nitz19,
	author = {A.H. Nitz and others},
	journal = {Astrophys. J.},
	volume = {891},
	pages = {123},
	year = {2019}
}

@article{Nitz20,
	author = {A.H. Nitz and others},
	journal = {Astrophys. J.},
	volume = {897},
	pages = {2},
	year = {2020}
}

@article{Owen99,
	author = {B.J. Owen and others},
	journal = {Phys. Rev. D},
	volume = {60},
	pages = {022002},
	year = {1999}
}

@article{Pretorius05,
	author = {Frans Pretorius},
	journal = {Class. Quantum Grav.},
	volume = {22},
	pages = {425},
	year = {2005}
}

@book{Rabiner10,
	author = {Rabiner, R. and Schafer, R.},
	title = {Theory and Applications of Digital Speech Processing},
	publisher = {Prentice Hall Press},
	address = {United States},
	year = {2010}
}

@article{Razzano18,
	author = {M. Razzano and others},
	journal = {Class. Quantum Grav.},
	volume = {35},
	pages = {095016},
	year = {2018}
}

@article{Russo14,
	author = {M. Russo and others},
	journal = {Solar Energy},
	volume = {105},
	pages = {264},
	year = {2014}
}

@article{Russo16,
	author = {M. Russo},
	journal = {Swarm. Evo. Comp.},
	volume = {27},
	pages = {145},
	year = {2016}
}

@article{Russo20,
	author = {M. Russo},
	journal = {Soft Comp.},
	volume = {24},
	pages = {16885},
	year = {2020}
}

@article{Russo00,
	author = {M. Russo},
	journal = {IEEE Trans. Evo. Comput.},
	volume = {4},
	year = {2000}
}

@article{Sylvestre02,
	author = {J. Sylvestre and others},
	journal = {Phys. Rev. D},
	volume = {66},
	pages = {102004},
	year = {2002}
}

@article{Usman16,
	author = {S.A. Usman and others},
	journal = {Class. Quant. Grav.},
	volume = {33},
	pages = {215004},
	year = {2016}
}

@article{Venumadhav20,
	author = {T. Venumadhav and others},
	journal = {Phys. Rev. D},
	volume = {101},
	pages = {083030},
	year = {2020}
}

%%%%%%%%
%%%%%%%%
%%%%%%%%
% Speech processing

@article{Beritelli97,
	author = {F. Beritelli and S. Casale and A. Cavallaro},
	journal = {Electron. Lett.},
	volume = {33},
	pages = {1846},
	year = {1997}
}

@article{Beritelli98,
	author = {F. Beritelli and S. Casale and A. Cavallaro},
	journal = {IEEE J. Sel. Areas Comm.},
	volume = {16},
	pages = {1818},
	year = {1998}
}

@article{Beritelli99,
  author = {F. Beritelli and S. Casale and M. Russo},
  journal = {Int. J. of Patt. Rec. Artif. Int.},
  year = {1999},
  volume = {13},
  pages = {109--132}
}

